AdaptiveRec: Adaptively Construct Pairs for Contrastive Learning in Sequential Recommendation

This paper presents a solution to the challenges faced by contrastive learning in sequential recommendation systems. In particular, it addresses the issue of false negative, which limits the effectiveness of recommendation algorithms. By introducing an advanced approach to contrastive learning, the proposed method improves the quality of item embeddings and mitigates the problem of falsely categorizing similar instances as dissimilar. Experimental results demonstrate performance enhancements compared to existing systems. The flexibility and applicability of the proposed approach across various recommendation scenarios further highlight its value in enhancing sequential recommendation systems.

==> temp.tex <==
%chap2 content : related works
\section{Contrastive Learning}
Contrastive learning is a type of self-supervised learning technique, where the goal is to learn useful representations of data without any explicit labeling or supervision\cite{le2020contrastive}.
In contrastive learning, the algorithm is trained to compare and contrast different samples of data to learn the underlying patterns and relationships between them.
The basic idea is to take two different data points and generate two different representations for each data point\cite{oord2018representation}.
The algorithm aims to learn to differentiate between representations of the same data point, referred to as a positive pair, and representations of different data points, known as a negative pair, using a similarity metric.
The training process involves optimizing the model to maximize the similarity between the representations of positive pairs while minimizing the similarity between the representations of negative pairs.
This way, the model learns to capture the meaningful differences and similarities between the data points, which can then be used for downstream tasks such as classification, clustering, or retrieval.

Contrastive learning can be mathematically formulated using the InfoNCE (Normalized Mutual Information Neural Estimation)\cite{wu2022infocse} loss function, which is used to maximize the similarity between positive pairs and minimize the similarity between negative pairs.
The InfoNCE loss is defined as:
\begin{equation}\label{eq:infoNCE}
\ell_\mathsf{NCE} 
\triangleq \mathop{\mathbb{E}}\limits_{\substack{(x,x^+) \sim p_\mathsf{pos}\\
\{x_i^-\}_{i=1}^M\overset{{i.i.d.}}{\sim}p_\text{data}}}
\Bigg[ -\text{log} \frac{e^{f(x)^\top f(x^+)/\tau}}{e^{f(x)^\top f(x^+)/\tau} + \sum_i e^{f(x_i^-)^\top f(x)/\tau}} \Bigg]
\end{equation}

\subsection{Contrastive Learning in Sentence Embedding}
% SimCSE
The paper introduces SimCSE\cite{gao2021simcse} a contrastive sentence embedding framework, which utilizes pre-trained embeddings to enhance the quality of sentence representations.
It employs contrastive learning principles to bring similar samples closer and push dissimilar samples apart, resulting in improved uniformity and alignment within the embeddings.
The paper presents two variations: unsupervised SimCSE, which introduces dropout-based noise\cite{srivastava2014dropout} and batch-level negative sampling, and supervised SimCSE\cite{gao2021simcse}, which utilizes NLI(Natural Language Inference) datasets with entailment and contradiction pairs\cite{conneau2017supervised}\cite{reimers2019sentence}. 
Therefore, for each premise and its entailment hypothesis, there is an accompanying contradiction
hypothesis7

Both variations demonstrate the effectiveness of contrastive objectives in refining sentence embeddings.
SimCSE\cite{gao2021simcse} offers a promising approach to enhance the quality of sentence representations, making it applicable to various natural language processing tasks.\\

% DiffCSE
DiffCSE\cite{chuang2022diffcse} is an extension of SimCSE\cite{gao2021simcse} that addresses limitations in the unsupervised learning domain by considering additional augmentation methods and promoting equivariant contrastive learning\cite{dangovski2021equivariant} for sentence embeddings.
While SimCSE\cite{gao2021simcse} focuses on dropout insensitivity, DiffCSE\cite{chuang2022diffcse} argues for sensitivity to augmentation techniques like masked language models.
Leveraging theoretical foundations from computer vision, DiffCSE\cite{chuang2022diffcse} emphasizes the superiority of equivariant contrastive learning, surpassing the limited capabilities of invariance-based approaches.
It incorporates a difference prediction objective using a conditional ELECTRA\cite{clark2020electra} architecture to capture distinctions between original and modified sentences.
By broadening augmentation methods and embracing equivariant contrastive learning, DiffCSE\cite{chuang2022diffcse} enhances the robustness of sentence embeddings in unsupervised learning, providing valuable insights for more sophisticated representation learning frameworks in natural language processing.\\

% PromCSE

PromCSE\cite{jiang2022improved} incorporates an Energy-based Hinge loss, leveraging hard negatives for improved discrimination in supervised learning.
The inclusion of this loss enhances the model's ability to distinguish between similar and dissimilar sentences, surpassing softmax-based losses.
PromCSE's\cite{jiang2022improved} integration of frozen PLMs, Soft Prompts, and the Energy-based Hinge loss provides a compelling approach to address overfitting and domain shift, advancing deep learning in natural language processing tasks.\\

\subsection{Contrastive Learning in Sequential Recommendation}
% SASRec, BERT4Rec
% next item prediction task에 기반하고 있다. \\

% CL4SRec
Contrastive Learning for Sequential Recommendation\cite{xie2022contrastive} is proposed as a solution to address the significant issue of data sparsity in recommendation systems by incorporating contrastive learning techniques.
CL4SRec\cite{xie2022contrastive} focuses on constructing pairs with different viewpoints, where positive pairs carry semantic information.
The paper introduces three data augmentation techniques at the sequence level to obtain more effective user representations. These augmentation methods include item cropping, which involves cropping a certain interval within the sequence, item masking, which masks several items within the sequence, and item reordering, which rearranges the order of items within a specific interval in the sequence.
By applying these data augmentation techniques, CL4SRec\cite{xie2022contrastive} performs contrastive learning by creating positive pairs from the original sequence.
These augmentation methods closely resemble the data augmentation approaches commonly used in the field of computer vision.\cite{chen2020simple}
This integration of contrastive learning and sequence-based data augmentation in CL4SRec\cite{xie2022contrastive} contributes to advancements in addressing data sparsity and enhancing sequential recommendation systems.\\

% DuoRec
DuoRec\cite{qiu2022contrastive} model combines two forms of contrastive loss.
Firstly, it utilizes unsupervised augmentation through dropout-based model-level augmentation to create positive pairs.
It emphasizes the importance of pairing samples under the assumption that their meaning remains unchanged.
The paper also highlights that semantic preservation alone in CL4SRec\cite{xie2022contrastive} may not be sufficient.
In this regard, the proposed DuoRec\cite{qiu2022contrastive} model heavily incorporates the feature-level augmentation through dropout, as suggested by SimCSE\cite{gao2021simcse}. Additionally, DuoRec\cite{qiu2022contrastive} employs supervised positive sampling, where pairs are created by considering sequences with the same target item as positive samples.
This approach enhances the model's ability to capture the relationships between sequences with shared target items.
By combining both unsupervised and supervised contrastive learning, DuoRec\cite{qiu2022contrastive} aims to improve the effectiveness of recommendation models in capturing semantic information and considering item-level relationships.\\

% ECL-SR

\subsection{Alignment and Uniformity}
In order to point out how well features are represented, previous work has suggested two key properties; alignment and uniformity\cite{wang2020understanding}.
Alignment measures how well paired positive instances are closely represented, typically computed as the average distance between them.
On the other hand, uniformity assesses how well the feature distribution is uniformly spread, often quantified using a Gaussian kernel on a hypersphere.
Given the data distribution $p_{data}$ and a positive pair distribution $p_{pos}$, alignment and uniformity is defined as : 

\begin{equation}\label{eq:align} \ell_{\text{align}} \triangleq \mathbb{E}_{(x,x^+) \sim p_{\text{pos}}} \| f(x) - f(x^+) \|^2 \end{equation}
\begin{equation}\label{eq:uniform} \ell_{\text{uniform}} \triangleq \mathbb{E}_{(x,y) \sim p_{\text{data}}} e^{-2 \| f(x) - f(y) \|^2} \end{equation}

Minimizing both metrics indicates an improved performance.
Minimizing $\ell_{\text{align}}$ in equation \ref{eq:align} encourages the learned representations of samples $x$ and $x^+$, sampled from $p_{\text{pos}}$, to be closer together.
Minimizing $\ell_{\text{uniform}}$ in euation \ref{eq:uniform} encourages the samples from $p_{\text{data}}$ to be uniformly represented.
By considering these two objectives, the goal is to enhance the proximity of positive pairs while promoting uniform representation across the data distribution.
